Enhanced ASR Robustness to Packet Loss with a Front-End Adaptation Network

In the realm of automatic speech recognition (ASR), robustness in noisy environments remains a significant challenge. Recent ASR models, such as Whisper, have shown promise, but their efficacy in noisy conditions can be further enhanced. This study is focused on recovering from packet loss to improve the word error rate (WER) of ASR models. We propose using a front-end adaptation network connected to a frozen ASR model. The adaptation network is trained to modify the corrupted input spectrum by minimizing the criteria of the ASR model in addition to an enhancement loss function. Our experiments demonstrate that the adaptation network, trained on Whisper's criteria, notably reduces word error rates across domains and languages in packet-loss scenarios. This improvement is achieved with minimal affect to Whisper model's foundational performance, underscoring our method's practicality and potential in enhancing ASR models in challenging acoustic environments.

==> extra.tex <==


% \begin{table}[ht]
% \centering
% \caption{Comparison of WER\%for Different Loss Function Configurations on the ALLSTAR dataset using the whisper base model}
% \begin{tabular}{c c|c }
% \hline
% Packet loss rate & Loss function & WER\% \\
% \hline
% \multirow{4}{*}{0\%} & Whisper & \textbf{0.222}  \\
%                      & Ours     & 0.227  \\
%                      & L1 only     & 0.227  \\
%                      & CE only     & 0.227 \\
% \hline
% \multirow{4}{*}{10\%}& Whisper & \textbf{0.222}  \\
%                      & Ours     & 0.227  \\
%                      & L1 only     & 0.227  \\
%                      & CE only     & 0.227 \\
% \hline
% \multirow{4}{*}{20\%} & Whisper & \textbf{0.222}  \\
%                      & Ours     & 0.227  \\
%                      & L1 only     & 0.227  \\
%                      & CE only     & 0.227 \\
% \hline
% \multirow{4}{*}{30\%} & Whisper & \textbf{0.222}  \\
%                      & Ours     & 0.227  \\
%                      & L1 only     & 0.227  \\
%                      & CE only     & 0.227 \\
% \hline
% \multirow{4}{*}{40\%} & Whisper & \textbf{0.222}  \\
%                      & Ours     & 0.227  \\
%                      & L1 only     & 0.227  \\
%                      & CE only     & 0.227 \\
% \hline
% \end{tabular}
% \label{table:wer_loss_function}
% \end{table}


% \begin{table}[ht]
% \centering
% \caption{Comparison of WER\% for other PLC, L1 and CE, and Baseline Scenarios}
% \begin{tabular}{|c c|}
% \hline
% Scenario & WER\% \\
% \hline
% Other PLC & 1.022 \\
% L1 and CE & 0.237 \\
% Whisper & 0.219 \\
% \hline
% \end{tabular}
% \label{table:wer_scenario_snr_}
% \end{table}






% \begin{table}[ht]
% \centering
% \caption{Comparison of WER\% and Hallucination Rate for Different PL Rates}
% \begin{tabular}{|c c|c c|}
% \hline
% Packet loss rate & Model & WER\% & Hallucination Rate \\
% \hline
% \multirow{3}{*}{0\%} & Whisper & \textbf{0.222} & [Your Value] \\
%                      & Ours     & 0.227 & [Your Value] \\
%                      & Other PLC     & 0.227 & [Your Value] \\
% \hline
% \multirow{3}{*}{5\%} & Whisper & \textbf{0.219} & [Your Value] \\
%                      & Ours     & 0.237 & [Your Value] \\
%                      & Other PLC      & 0.237 & [Your Value] \\
% \hline
% \multirow{3}{*}{10\%} & Whisper & 0.137 & [Your Value] \\
%                       & Ours     & 0.227 & [Your Value] \\
%                       & Other PLC      & 0.227 & [Your Value] \\
% \hline
% \multirow{3}{*}{20\%} & Whisper & 0.129 & [Your Value] \\
%                       & Ours     & \textbf{0.122} & [Your Value] \\
%                       & Other PLC      & 0.227 & [Your Value] \\
% \hline
% \multirow{3}{*}{30\%} & Whisper & 0.171 & [Your Value] \\
%                       & Ours     & 0.095 & [Your Value] \\
%                       & Other PLC      & 0.227 & [Your Value] \\
% \hline
% \end{tabular}
% \label{table:wer_hallucination_model_variant_snr_comparison}
% \end{table}



